Non-invasive magnetocardiography of living rat based on diamond quantum sensor

Magnetocardiography (MCG) has emerged as a sensitive and precise method to diagnose cardiovascular diseases, providing more diagnostic information than traditional technology. However, the sensor limitations of conventional MCG systems, such as large size and cryogenic requirement, have hindered the widespread application and in-depth understanding of this technology. In this study, we present a high-sensitivity, room-temperature MCG system based on the negatively charged Nitrogen-Vacancy (NV) centers in diamond. The magnetic cardiac signal of a living rat, characterized by an approximately 20 pT amplitude in the R-wave, is successfully captured through non-invasive measurement using this innovative solid-state spin sensor. To detect these extremely weak biomagnetic signals, we utilize sensitivity-enhancing techniques such as magnetic flux concentration. These approaches have enabled us to simultaneously achieve a magnetometry sensitivity of 9 $\text{pT}\cdot \text{Hz}^{-1/2}$ and a sensor scale of 5 $\text{mm}$. By extending the sensing scale of the NV centers from cellular and molecular level to macroscopic level of living creatures, we have opened the future of solid-state quantum sensing technologies in clinical environments.

==> setuup.tex <==
Figure \ref{fig1}a and figure \ref{fig1}b demonstrates the setup of our diamond-based MCG system. 
The system is composed of several modules, including a microwave system, an optical system, an electronical acquisition system, together with some auxiliary equipments. 
All components are housed within a magnetic shielding cylinder made from multi-layer permalloy to suppress the electromagnetic noise in lab environment. 
A pair of saddle-like coils was wired in the shielding cylinder to provide bias field and calibration waveform. 
The rat was placed in a manual three-axis translation stage to adjust position and approach the diamond sensor in measurement. 


% 1. MW
The microwave system consists of two FSW-0010 sources which generate microwave signal at two different NV resonant frequencies to perform dual-resonance magnetometry. 
The two microwave outputs are modulated by the same optimized frequency of 21637 Hz with a $\pi$ phase shift produced by a signal generator, so that the demodulated PL signal from $\ket{m_s=+1}$ and $\ket{m_s=-1}$ states could reserve the common mode magnetic signal and eliminate the anti-common mode temperature signal. 
This dual-resonance magnetometry method was deployed to simultaneously manipulate the electron spin resonant levels $\ket{m_s=+1}$ and $\ket{m_s=-1}$ in external magnetic field, effectively minimizing the impact of temperature shift and improving the readout contrast for magnetic field, as illustrated in figure \ref{fig3}a. 
The two microwave signals are amplified and combined into the diamond through double-split ring radiation structure  as shown in figure \ref{fig1} c, allowing the NV centers to be manipulated. 

% 2. acq
In the development of the electronical acquisition system, we employed a phase-locked loop readout technique based on microwave frequency modulation method, which could effectively avoid the 1/f electronic noise. 
The microwave-modulated PL signal and reference laser signal are separately converted into photocurrent with two photodiodes(PD), and demodulated with a 2-channel lock-in amplifier HF2LI. The magnetic field-dependent PL signal  acquired by the lock-in amplifier is shown in figure \ref{fig2} a. 
A data acquistion card MPS-140401 was used to acquire the rat's skin electronic potential and perform ECG measurement by LEAD II configuration. 

% 3. optical
The optical system comprises of a laser excitation module and a fluorescence collection module. 
A 532-nm laser with output power 1.5 W is used to generate the green light and excite the NV centers in diamond.
The laser is sampled by a polarized beam splitter(PBS), which allows the laser's reference photoelectric signal to be acquired by the lock-in amplifier to cancel the laser power fluctuation. 
The laser beam was adjusted by several reflectors and focused with a spherical lens with focal length $f=20mm$ to achieve maximum laser power density in diamond. 
An NV diamond sample with size $1 mm\times1mm\times0.12mm$ was fabricated as the sensor of this system. The red PL emitted from the NV centers in diamond is collected by a PD. To enhance the sensitivity of the diamond magnetometr,  a pair of magnetic flux concentrators made from high magnetic permeability materials(1J85) was adopted to improve the sensitivity of the MCG system. 
% 磁通聚集器的详细信息？
The geometrics of the flux concentrators was evaluated to balance the cardiac signal's attenuation with distance and the amplification factor of the flux concentrators. 

% 4. benchmark
Before the animal experiment, we first assessed the background magnetic sensitivity of the magnetometer by conducting measurement without rat specimen. 
This result is presented in figure \ref{fig2}b, where we plotted the density noise spectrum of the demodulated PL signal under both resonance and non-resonance situations by applying Fourier transformation of the data. 
In the frequency range related to the rat's cardiac signal spectrum, which spans from 1 Hz to 200 Hz, the anticipated magnetic sensitivity is $9.25pT/\sqrt{Hz}$.
This result provides a benchmark for the following animal experiment. 
% In terms of stability, a 24-hour test showed high consistency in magnetic sensitivity.
